ChatGPT or A Silent Everywhere Helper: A Survey of Large Language Models

Large Language Models (LLMs) have revo lutionized natural language processing Natural Language Processing (NLP), with Chat Generative Pre-trained Transformer (ChatGPT) standing out as a notable exampledue to its advanced capabilities and widespread applications. This survey provides a comprehensive analysis of ChatGPT, exploring its architecture, training processes, and functionalities. We examine its integration into various domains across industries such as customer service, education, healthcare, and entertainment. A comparative analysis with other LLMs highlights ChatGPT's unique features and performance metrics. Regarding benchmarks, the paper examines ChatGPT's comparative performance against other LLMs and discusses potential risks such as misinformation, bias, and data privacy concerns. Additionally, we offer a number of figures and tables that outline the backdrop of the discussion, the main ideas of the article, the numerous LLM models, a thorough list of datasets used for pre-training, fine-tuning, and evaluation, as well as particular LLM applications with pertinent references. Finally, we identify future research directions and technological advancements, underscoring the evolving landscape of LLMs and their profound impact on artificial intelligence Artificial Intelligence (AI) and society.

==> 10_Acronyms.tex <==
\begin{acronym}
\newacronym{absa}{ABSA}{Aspect-Based Sentiment Analysis}
\newacronym{acc}{ACC}{Automatic Conversation}
\newacronym{ae}{AE}{autoencoding}
\newacronym{ai}{AI}{Artificial Intelligence}
\newacronym{albert}{ALBERT}{A Lite BERT}
\newacronym{api}{API}{Application Programming Interface}
\newacronym{ar}{AR}{autoregressive}
\newacronym{ape}{APE}{Absolute Positional Encoding}
\newacronym{asr}{ASR}{Automatic Speech Recognition}
\newacronym{ast}{AST}{Abstract Syntax Tree}
\newacronym{bart}{BART}{Bidirectional and Auto-Regressive Transformer}
\newacronym{bert}{BERT}{Bidirectional Encoder Representations from Transformers}
\newacronym{berf}{BERF}{BERT Random Fores}
\newacronym{biaffine}{Biaffine}{Biaffine Attention for Dependency Parsing}
\newacronym{bilstm}{BiLSTM}{Bidirectional Long Short-Term Memory}
\newacronym{bleu}{BLEU}{Bilingual Evaluation Understudy}
\newacronym{bleurt}{BLEURT}{Bilingual Evaluation Understudy with Representations from Transformer}
\newacronym{bpe}{BPE}{Byte Pair Encoding}
\newacronym{cap}{CAP}{Contrastive pruning}
\newacronym{cbt}{CBT}{Cognitive Behavioral Therapy}
\newacronym{clip}{CLIP}{Contrastive Language–Image Pre-training}
\newacronym{cls}{CLS}{Causal Language Modeling}
\newacronym{cnn}{CNN}{Convolutional Neural Network}
\newacronym{copa}{COPA}{Choice of Plausible Alternatives}
\newacronym{cot}{CoT}{Chain of Thought}
\newacronym{cpu}{CPU}{Central Processing Unit}
\newacronym{cr}{CR}{Comparative Ranking}
\newacronym{crf}{CRF}{Conditional Random Field}
\newacronym{csr}{CSR}{Conversational Speech Recognition}
\newacronym{ctc}{CTC}{Connectionist Temporal Classification}
\newacronym{cxl}{CXL}{Compute Express Link}
\newacronym{depn}{DEPN}{Detect and Editing Privacy Neurons}
\newacronym{dl}{DL}{Deep Learning}
\newacronym{dpo}{DPO}{Direct Preference Optimization}
\newacronym{drp}{DRP}{Deep Reinforcement Learning}
\newacronym{dst}{DST}{Dialogue State Tracking}
\newacronym{e2e}{E2E}{End-to-End}
\newacronym{eae}{EAE}{Event Argument Extraction}
\newacronym{ecqa}{ECQA}{Explanation and Commonsense Question Answering}
\newacronym{electra}{ELECTRA}{Efficiently Learning an Encoder that Classifies Token Replacements Accurately}
\newacronym{erc}{ERC}{Emotion Recognition in Conversation}
\newacronym{esb}{ESB}{Extended Summarization Benchmark}
\newacronym{factscore}{FactScore}{Fact Consistency Scoring}
\newacronym{flan}{FLAN}{Fine-tuned Language Net}
\newacronym{fnn}{FNN}{Feed-Forward Neural Network}
\newacronym{gpt}{GPT}{Generative Pre-trained Transformer}
\newacronym{gpu}{GPU}{Graphics Processing Unit}
\newacronym{gqa}{GQA}{General Question Answering}
\newacronym{hf}{HF}{Hugging Face}
\newacronym{iad}{IAD}{Industrial Anomaly Detection}
\newacronym{ids}{IDS}{Intrusion Detection System}
\newacronym{ilm}{ILM}{Instruction Learning Model}
\newacronym{iomt}{IoMT}{Internet of Medical Things}
\newacronym{iot}{IoT}{Internet of Things}
\newacronym{kd}{KD}{Knowledge Distillation}
\newacronym{kg}{KG}{Knowledge Graph}
\newacronym{laclip}{LaCLIP}{Language Augmented CLIP}
\newacronym{llama}{LLaMA}{Large Language Model Meta AI}
\newacronym{LLM}{LLM}{Large Language Model}
\newacronym{llvm-ad}{LLVM-AD}{Large Language and Vision Models for Autonomous Driving}
\newacronym{lm}{LM}{Language Model}
\newacronym{lpe}{LPE}{Learnable Positional Embedding}
\newacronym{lstm}{LSTM}{Long Short-Term Memory}
\newacronym{lvlm}{LVLM}{Large Vision-Language Model}
\newacronym{mad}{MAD}{Multiply-Add}
\newacronym{mc}{MC}{Multiple Classification}
\newacronym{meteor}{METEOR}{Metric for Evaluation of Translation with Explicit Ordering}
\newacronym{ml}{ML}{Machine Learning}
\newacronym{mllm}{MLLM}{Multimodal Large Language Model}
\newacronym{mlm}{MLM}{Masked Language Modeling}
\newacronym{moe}{MoE}{Mixture of Experts}
\newacronym{msmarco}{MS MARCO}{Microsoft MAchine Reading COmprehension}
\newacronym{mt}{MT}{Machine Translation}
\newacronym{ner}{NER}{Named Entity Recognition}
\newacronym{nlg}{NLG}{Natural Language Generation}
\newacronym{nli}{NLI}{Natural Language Inference}
\newacronym{nlp}{NLP}{Natural Language Processing}
\newacronym{nlu}{NLU}{Natural Language Understanding}
\newacronym{nsfw}{NSFW}{Not Safe For Work}
\newacronym{oov}{OOV}{Out-Of-Vocabulary}
\newacronym{opf}{OPF}{Optimal Power Flow}
\newacronym{otd}{OTD}{One True Dialogue}
\newacronym{owl}{OWL}{Outlier Weighed Layer-wise}
\newacronym{palm}{PaLM}{Pathways Language Model}
\newacronym{para}{PARA}{Paraphrase Identification}
\newacronym{peft}{PEFT}{Parameter Efficient Fine-Tuning}
\newacronym{plo}{PLO}{Posterior Log Odds}
\newacronym{pos}{PoS}{Part-of-Speech}
\newacronym{ppo}{PPO}{Proximal Policy Optimization}
\newacronym{ptm}{PTM}{Pre-trained Model}
\newacronym{ptq}{PTQ}{Post-Training Quantization}
\newacronym{qa}{QA}{Question Answering}
\newacronym{qaqg}{QAQG}{Question Answering Question Generation}
\newacronym{qat}{QAT}{Quantization-Aware Training}
\newacronym{raf}{RAF}{Reasoning Accuracy Framework}
\newacronym{rlhf}{RLHF}{Reinforcement Learning from Human Feedback}
\newacronym{rlaif}{RLAIF}{Reinforcement Learning from AI Feedback}
\newacronym{rm}{RM}{Reward Modeling}
\newacronym{roberta}{RoBERTa}{Robustly Optimized BERT Pre-training Approach}
\newacronym{rope}{RoPE}{Rotary Positional Embedding}
\newacronym{rouge}{ROUGE}{Recall-Oriented Understudy for Gisting Evaluation}
\newacronym{rpe}{RPE}{Relative Positional Encoding}
\newacronym{rnn}{RNN}{Recursive Neural Network}
\newacronym{rstb}{RSTB}{Residual Swin Transformer Block}
\newacronym{sa}{SA}{Surprise Adequacy}
\newacronym{sds}{SDS}{Spoken Dialogue System}
\newacronym{sft}{SFT}{Safety Fine-Tuning}
\newacronym{simd}{SIMD}{Single-Instruction Multiple-Data}
\newacronym{sld}{SLD}{Self-correcting Language-Driven}
\newacronym{smote}{SMOTE}{Synthetic Minority Over-sampling Technique}
\newacronym{sram}{SRAM}{Static Random Access Memory}
\newacronym{sst}{SST}{Sentiment Sentence Treebank}
\newacronym{strn}{STRN}{Swin Transformer and ResNet-based Generative Adversarial Network}
\newacronym{stu}{STU}{Source-Target Unification}
\newacronym{svm}{SVM}{Support Vector Machine}
\newacronym{t5}{T5}{Text-to-Text Transfer Transformer}
\newacronym{tapex}{TAPEX}{Tabular Pretraining for Data Extraction and eXploration}
\newacronym{tf-idf}{TF-IDF}{Term Frequency-Inverse Document Frequency}
\newacronym{thi}{THI}{Tinnitus Handicap Inventory}
\newacronym{tgi}{TGI}{Textual Generative Intelligence}
\newacronym{tip}{TIP}{Topic-based Information Prioritization}
\newacronym{tpu}{TPU}{Tensor Processing Unit}
\newacronym{ts}{TS}{Token Similarity}
\newacronym{tts}{TTS}{Text-to-Speech}
\newacronym{vqa}{VQA}{Visual Question Answering}
\newacronym{wsd}{WSD}{Word Sense Disambiguation}
\newacronym{xglue}{XGLUE}{Cross-lingual General Language Understanding Evaluation}
\newacronym{glue}{GLUE}{General Language Understanding Evaluation}
\end{acronym}

==> 4_Resource_of_LLMs.tex <==
\section{Resource of LLMs}\label{resource}
\begin{figure*}[!htb]
    \centering
    \includegraphics[width=.84\linewidth]{Resource of LLM_new.pdf}
    \caption{Various LLM Datasets}
    \label{resource_LLM}
\end{figure*}
The resources required for developing and deploying~\acp{LLM} are extensive and multifaceted~(See Fig. ~\ref{resource_LLM}). They include:\\
1. Computational Resources~\cite{hadi2023survey, zhao2023best}\\
\begin{itemize}
    \item High-Performance~\acp{GPU}/\acp{TPU}: Essential for training large models, examples include NVIDIA A100, V100, and Google's~\acp{TPU}.\\
    \item High-Performance Computing Clusters: Large-scale clusters to distribute the computational load.\\
    \item Cloud Computing Services: Providers like~\ac{AWS}, Google Cloud, and Microsoft Azure offer scalable infrastructure.\\
\end{itemize}
2. Data Resources~\cite{zhang2023large}\\
\begin{itemize}
    \item Diverse and Large Datasets: Datasets like Common Crawl, Wikipedia, The Pile, and more. Date will be explained with details in the next section.\\
    \item Data Storage and Management: Large-scale storage solutions to handle and process massive datasets.\\
    \item Data Preprocessing Tools: Tools and software for cleaning, organizing, and preparing data for training.\\
\end{itemize}
3. Human Resources\\
\begin{itemize}
    \item Expert Researchers and Engineers: Specialists in machine learning, natural language processing, and data science.\\
    \item Annotation and Labeling Teams: For supervised learning tasks, human annotators are needed to label data.\\
\end{itemize}
4. Software Resources~\cite{roffo2024exploring}\\
\begin{itemize}
    \item Machine Learning Frameworks: Libraries like TensorFlow, PyTorch, JAX, and Keras.\\
    \item Pretrained Models and Transfer Learning: Models such as~\ac{GPT}-3,~\ac{BERT}, and T5, which can be fine-tuned for specific tasks.\\
\end{itemize}
5. Financial Resources\\
\begin{itemize}
    \item Funding for Research and Development: Significant investment is required for hardware, software, and human capital.\\
    \item Operational Costs: Ongoing costs for cloud services, data storage, and utilities.
\end{itemize}
6. Infrastructure Resources\\
\begin{itemize}
    \item Data Centers: Physical locations housing the computational and storage infrastructure.\\
    \item Network Connectivity: High-speed internet connections to facilitate data transfer and distributed computing.\\
\end{itemize}
7. Ethical and Regulatory Resources\\
\begin{itemize}
    \item Ethics Committees and Review Boards: To ensure responsible~\ac{AI} development.\\
    \item Legal and Compliance Teams: To navigate data privacy laws and regulations.\\
\end{itemize}
8. Collaboration and Community Resources\\
\begin{itemize}
    \item Research Collaborations: Partnerships with academic institutions and industry leaders.\\
    \item Open Source Communities: Contributions to and from open-source projects and repositories.\\
    \item These resources collectively enable the development, training, and deployment of~\acp{LLM}, allowing them to perform a wide array of tasks across different domains.\\
\end{itemize}



==> 8_Future_Directions_and_Open_Research_Areas.tex <==
\section{Future Directions and Open Research Areas}\label{future}

==> acronyms1.tex <==
\newacronym{LLM}{Large Language Model}{Large Language Model}

